A hybrid approach to supervised machine learning for algorithmic melody composition

In this work we present an algorithm for composing monophonic melodies similar in style to those of a given, phrase annotated, sample of melodies. For implementation, a hybrid approach incorporating parametric Markov models of higher order and a contour concept of phrases is used. This work is based on the master thesis of Thayabaran Kathiresan (2015). An online listening test conducted shows that enhancing a pure Markov model with musically relevant context, like count and planed melody contour, improves the result significantly.

==> latex_einstellungen/abkuezungen/abkuerzungen.tex <==
\nomenclature{CSP}{Constraint satisfaction problem}
\nomenclature{CBR}{Case based reasoning}

\nomenclature{UGC}{User Generated Content}
\nomenclature{CSS}{Cascading Style Sheets}
\nomenclature{JS}{JavaScript}
\nomenclature{SQL}{Structured Query Language}
\nomenclature{GPL}{GNU General Public License}
\nomenclature{GNU}{GNU is not Unix}
\nomenclature{LGPL}{GNU Lesser General Public License}
\nomenclature{XMPP}{Extensible Messaging and Presence Protocol}
\nomenclature{IM}{Instant Message}
\nomenclature{CMS}{Content Management System}
\nomenclature{RSS}{Really Simple Syndication}
\nomenclature{JSON}{JavaScript Object Notation}
\nomenclature{HTML}{Hypertext Markup Language}
\nomenclature{TDD}{Test-driven development}
\nomenclature{GUI}{Graphical User Interface}
\nomenclature{KPI}{Key Performance Indicator}
\nomenclature{WWW}{World Wide Web}
\nomenclature{OCR}{Optical Character Recognition}
\nomenclature{ERM}{Entity Relationship Modell}

